Distributional Reinforcement Learning for Energy-Based Sequential Models

Global Autoregressive Models (GAMs) are a recent proposal [Parshakova et al., CoNLL 2019] for exploiting global properties of sequences for data-efficient learning of seq2seq models. In the first phase of training, an Energy-Based model (EBM) over sequences is derived. This EBM has high representational power, but is unnormalized and cannot be directly exploited for sampling. To address this issue [Parshakova et al., CoNLL 2019] proposes a distillation technique, which can only be applied under limited conditions. By relating this problem to Policy Gradient techniques in RL, but in a \emph{distributional} rather than \emph{optimization} perspective, we propose a general approach applicable to any sequential EBM. Its effectiveness is illustrated on GAM-based experiments.

==> ExperimentsAndResults.tex <==


\begin{outline}[itemize]
\1 \MD{What are the most important things to convey to the reader in my opinion:
    \2 The reader should understand the data efficiency aspects (easy)
    \2 RS vs Snis and especially Distill vs DPG should be illustrated (easy)
    \2 If possible, $P_\lambda$ and moments should be illustrated. For that purpose and for general reader understanding, it would be useful to have the "illustration" of CONLL-Table 2 somewhere. Could we just use it directly? But no D-PG results there... (issue here ?)
    \2 The fact that DPG works as expected (namely, approximates well the given P) is the most important thing to stress 
}

\1 \MD{Main issues}
    \2 While several of the plots are very nice and convey the ideas adequately, we have more difficulty with which statistics to present
    \2 We can put some of the tables in the SupMat, but we should have a couple of tables in the main text
        \3 If possible, one table that conveys the idea that our observations are not cherry-picked, but have some statistical validity: perhaps Fig 4 ??? \TA{why figure 4? Distillation: same seed, different motifs?} \MD{Not sure, the best would be to have one table that summarizes the overall statistics, including  dpg, and convinces the reader of its statistical validity. Fig 4 does not do that , but appears to correspond to many experiments...  What would you suggest?}
        \3 One table to compare distill and dpg: Fig 23 or 22  But will the reviewer be convinced of the statistical validity ? (see also my question below relative to these figs)
        

\1 \MD{In terms of a four-panel figure similar to CONLL-Fig-2, perhaps do a four-panel fig from AAAI-Previous-Figs-1-and-6 \TA{we also have figure 15 and 16}?. If I am correct, they correspond to the same motif, and illustrate distillation vs D-PG.}\TA{yes}
    \2 Can be used for explaining: data-efficiency; rs vs snis in training-1; distill vs DPG in training-2

    \2 We can then use this same figure to comment on the main findings: data-efficiency, rs vs snis (only in Fig-1, is this a pb?), distill vs D-PG. Question: Fig 6 is using snis or rs for Training-1 ?\TA{i think so too}
    
    \2 However, a four panel takes a lot of space. If too much, then use only one motif ?

\1 Ability of D-PG to work well. Figure 12 can be exploited for that:
    \2 We see that WN-DPG is good
    \2 But also that dpg-pi closely follows p-lambda \emph{(??: QUESTION: I am confused about the lines dpg-p-lambda and dpg-pi: does one of these lines correspond to the CE for p-lambda ?? )} \TA{well, dpg p-lambda and dpg pi are inside the cross entropy box, hence they both correspond to CE}
    \MD{I mean: i do not understand the difference between dpg-p-lambda and dpg-pi; i was hoping that dpg-p-lambda actually corresponds to p-lambda, implying that dpg-pi approximates p-lambda very well, an important message to convey if true}

\1 \MD{More on Statistics}
    \2 \MD{Figs 22 and 23}
        \3 \MD{Please explain the difference. In your comments, under "statistics/ d-pg", you mention that you did most of the experiments for a single motif in dpg, but not for distill, but Figs 22-23 mention three motifs ...} \TA{for the stats tables distillation and d-pg have almost the same number of experiments, but d-pg has a bit less. i mean, not the full number of all possible combinations}

\1 \MD{Length feature: Experiments should be mentioned briefly in the text, but Figure(s) and Table(s) should be placed in the SupMat.}

\1 \MD{PG vs D-PG: only mention difference briefly in text; possibly actually better to do it in the model section!}

\end{outline}



\section{Experiments}
\subsection{Plan of experiments}
\begin{itemize}
    \item Fixed: length = 30
    \item Fixed: one motif feature, fixed distractors 
    \item Variable: two length features - separate experiment that exploits these features, in the rest of experiments they are absent
    \item Variable: motif, D size, seed
\end{itemize}
\subsection{Cross entropy of $\pi_\theta$ depending on $|D|$}
\subsection{Distillation}
            
            
\begin{figure}[h]
    \centering
    \includegraphics[ width=0.7\linewidth]{figures/ce_freq_distill_m1s2.pdf} 
    \caption{\label{f:distill_m1s2} Distillation: different seeds, same motif}
\end{figure}
       
\begin{figure}[h]
    \centering
    \includegraphics[ width=1.0\linewidth]{figures/distill_m1s2.PNG} 
    \caption{\label{ft:distill_m1s2} Distillation: different seeds, same motif}
\end{figure}
            
\begin{figure}[h]
    \centering
    \includegraphics[ width=0.7\linewidth]{figures/ce_freq_distill_m2s1.pdf} 
    \caption{\label{f:distill_m2s1} Distillation: same seed, different motifs}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[ width=1.0\linewidth]{figures/distill_m2s1.PNG} 
    \caption{\label{ft:distill_m2s1} Distillation: same seed, different motifs}
\end{figure}
            
\begin{itemize}
    \item see \figurename~\ref{f:distill_m1s2},~\ref{ft:distill_m1s2},~\ref{f:distill_m2s1},~\ref{ft:distill_m2s1}
    \item Training-1: SNIS and RS are very similar, while SNIS is more general
    \item for a small dataset size $|D|$, there is a big gap between the CE of $r(x)$ and the CE of $\pi_\theta(x)$. As $|D|$ increases
    \item these CE get closer to one another, but a large gap persists for $|D| = 5000$
    \item the relationship is mirrored in the motif frequency case as well
    \item when $p_\lambda$ is ideal (this is the case when $|D|$ is big, because $r$ is close to the true $p$ and learning $\lambda$ for matching moments is easy), then the distillation produces perfect AM
\end{itemize}
          
\subsection{D-PG}

\begin{figure}[h]
    \centering
    \includegraphics[ width=1.0\linewidth]{figures/dpg_m1s2.PNG} 
    \caption{\label{ft:dpg_m1s2} D-PG: different seeds, same motif}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[ width=0.7\linewidth]{figures/ce_freq_dpg_m1s2.pdf} 
    \caption{\label{f:dpg_m1s2} D-PG: different seeds, same motif}
\end{figure}
       

            
\begin{figure}[h]
    \centering
    \includegraphics[ width=0.7\linewidth]{figures/ce_freq_dpg_m2s1.pdf} 
    \caption{\label{f:dpg_m2s1} D-PG: same seed, different motifs}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[ width=1.0\linewidth]{figures/dpg_m2s1.PNG} 
    \caption{\label{ft:dpg_m2s1} D-PG: same seed, different motifs}
\end{figure}
            
\begin{itemize}
    \item see \figurename~\ref{f:dpg_m1s2},~\ref{ft:dpg_m1s2},~\ref{f:dpg_m2s1},~\ref{ft:dpg_m2s1}
    \item same as for the distillation casse: for a small dataset size $|D|$, there is a big gap between the CE of $r(x)$ and the CE of $\pi_\theta(x)$
    \item the relationship is mirrored in the motif frequency case as well
    \item when $p_\lambda$ is ideal (when $P_\lambda=wn(x)\cdot F(x)$), then the D-PG produces perfect AM, see Section D-PG and true $P(x)=wn(x) \cdot F(x)$
\end{itemize}

\subsection{the weakness of pure PG in minimizing CE}

\begin{figure}[h]
    \centering
    \includegraphics[ width=1.0\linewidth]{figures/dpg_pg_m1s1.PNG} 
    \caption{\label{ft:dpg_pg} D-PG vs PG: same seed, same motif}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[ width=0.7\linewidth]{figures/ce_freq_dpg_pg.pdf} 
    \caption{\label{f:dpg_pg} D-PG vs PG: same seed, same motif}
\end{figure}
\begin{itemize}
    \item see \figurename~\ref{f:dpg_pg},~\ref{ft:dpg_pg}
    \item PG does not improve the cross-entropy while D-PG does
    \item PG ends up producing sequences of length 2: $\langle BOS\rangle \langle EOS\rangle$
\end{itemize}


\subsection{ D-PG and true $P(x)=wn(x) \cdot F(x)$ }

\begin{figure}[h]
    \centering
    \includegraphics[ width=1.0\linewidth]{figures/dpg_wndpg.PNG} 
    \caption{\label{ft:dpg_wndpg} D-PG vs WN D-PG}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[ width=0.7\linewidth]{figures/ce_freq_dpg_wdpg.pdf} 
    \caption{\label{f:dpg_wndpg} D-PG vs WN D-PG}
\end{figure}

            
\begin{itemize}
    \item see \figurename~\ref{f:dpg_wndpg},~\ref{ft:dpg_wndpg}
    \item when given a true $P_\lambda$, then D-PG produces perfect AM
    \item when $|D|$ is small then the loglinear term in GAMs cannot compensate for bad $r$
    \item $CE(T, p_\lambda)$ computed by importance sampling
     \item Can confirm that $CE(T, \pi_\theta) \approx CE(T, p_\lambda)$
     \item both $CE(T, \pi_\theta), CE(T, p_\lambda)$ are visualised on the figures
\end{itemize}



\subsection{Distillation vs D-PG}

\begin{figure}[h]
    \centering
    \includegraphics[ width=1.0\linewidth]{figures/dpg_distill_m1s2.PNG} 
    \caption{\label{ft:dpg_distill_m1s2} D-PG vs Distillation: different seeds, same motif}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[ width=0.7\linewidth]{figures/ce_freq_distil_dpg_m1s2.pdf} 
    \caption{\label{f:dpg_distill_m1s2} D-PG vs Distillation: different seeds, same motif}
\end{figure}
       

            
\begin{figure}[h]
    \centering
    \includegraphics[ width=0.7\linewidth]{figures/ce_freq_distil_dpg_m2s1.pdf} 
    \caption{\label{f:dpg_distill_m2s1} D-PG vs Distillation: same seed, different motifs}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[ width=1.0\linewidth]{figures/dpg_distill_m2s1.PNG} 
    \caption{\label{ft:dpg_distill_m2s1} D-PG vs Distillation: same seed, different motifs}
\end{figure}
            
\begin{itemize}
    \item see \figurename~\ref{f:dpg_distill_m1s2},~\ref{ft:dpg_distill_m1s2},~\ref{f:dpg_distill_m2s1},~\ref{ft:dpg_distill_m2s1}
    \item D-PG and Distillation have same trends and are competitive
    \item for these particular experiments (these seeds and these motifs) the CE of distillation is a bit better than for D-PG, while the motif frequency relationship is reversed
\end{itemize}


\subsection{Length Features}

\begin{figure}[h]
    \centering
    \includegraphics[ width=1.0\linewidth]{figures/dpg_distill_len_nolen.PNG} 
    \caption{\label{ft:dpg_distill_len_rat} D-PG vs Distillation: length feature off or on ratios }
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[ width=0.7\linewidth]{figures/ce_freq_distil_dpg_m1s1_len_nolen.pdf} 
    \caption{\label{f:dpg_distill_len} D-PG vs Distillation: length feature on or off}
\end{figure}
       

\begin{figure}[h]
    \centering
    \includegraphics[ width=1.0\linewidth]{figures/dpg_distill_len_nolen_vals.PNG} 
    \caption{\label{ft:dpg_distill_len_val} D-PG vs Distillation: length feature on or off }
\end{figure}
            
\begin{itemize}
    \item see \figurename~\ref{f:dpg_distill_len},~\ref{ft:dpg_distill_len_rat},~\ref{ft:dpg_distill_len_val}
    \item the performance of two training set ups (Distillation and D-PG) are rather similar when the length feature is on or off
    \item $ft=1001111$ vs $ft=Mv1001111$
    \item length feature (has two components: $\frac{|x|}{\textrm{max\_len}}$ $M$ and $\frac{|x|^2}{\textrm{max\_len}^2}$ $v$) has different nature from the independent binary features, but it does not make the performance worse
    \item perhaps to see the impact of the length feature, the length of strings should be longer than 30
\end{itemize}

\subsection{Statistics}

\begin{figure}[h]
    \centering
    \includegraphics[ width=1.0\linewidth]{figures/stats_distill.PNG} 
    \caption{\label{ft:stats_distill} Statistics: Distillation }
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[ width=1.0\linewidth]{figures/stats_dpg.PNG} 
    \caption{\label{ft:stats_dpg} Statistics: D-PG  }
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[ width=1.0\linewidth]{figures/stats_distill_dpg.PNG} 
    \caption{\label{ft:stats_dpg_distill} Statistics: D-PG vs Distillation (ratio of means)}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[ width=1.0\linewidth]{figures/stats_distill_dpg_val.PNG} 
    \caption{\label{ft:stats_dpg_distill_val} Statistics: D-PG vs Distillation}
\end{figure}

\begin{itemize}
    \item see \figurename~\ref{ft:stats_distill},~\ref{ft:stats_dpg},~\ref{ft:stats_dpg_distill},~\ref{ft:stats_dpg_distill_val}
    \item means and standard deviations for experiments while changing seeds, features and motifs
    \item distillation: same behavior as in plots, when $|D|$ increases then $\pi_\theta$ CE is getting closer to the theoretical one; outperforms r in small conditions of $|D|$ in terms of motif frequency and CE
    \item d-pg: because I did most of the experiments for $motif=10001011111000$, in the stats table $CE(T, \pi_\theta(D_{500}))<CE(T, \pi_\theta(D_{1000}))$, for this particular motif, but is distillation there was more variety
\end{itemize}




==> introduction.tex <==
\section{Introduction}

In the last few years, neural sequential models have become mainstream in such NLP tasks as language modeling, natural language generation, machine translation, dialogue modeling, speech recognition. The dominant paradigm has been to train these text generation models in an \emph{autoregressive} way, that is, by directly conditioning the probability of the next symbol on the sequence prefix generated so far, and by minimizing the perplexity of training sequences relative to the resulting incremental generative process. Some well-known instances of this approach are LSTM-based \cite{SutskeverVL14} and Transformer-based \cite{Vaswani} decoders.

In RL terminology, such incremental processes can be identified with \emph{policies}, with states corresponding to prefix generated so far, and actions to selection of next symbol. And then, standard autoregressive training can be seen as a form of \emph{imitation learning}, with the next training symbol providing a direct supervision signal for training the policy. This approach has the advantage of simplicity, but several drawbacks: reliance on large training datasets, brittleness in front of test conditions deviating from training examples, inability to account for global consistency constraints on generated sequences.%
\MDEN{A bit verbose; ``exposure bias'', provide some examples?: duplication, inconsistency in chit-chat dialogue, program generation, ...}

Reinforcement learning differs from imitation learning by considering \emph{rewards}, which assess the global value of a decision sequence. A central problem is then to determine optimal policies, that is, policies that maximize reward expectation relative to environmental responses. Such approaches have been employed also for sequence generation problems, for such applications as machine translation \cite{DBLP:journals/corr/RanzatoCAZ15,bahdanau_actor-critic_2016} musical score generation \cite{Jaques-2017}, and many others. Such problems simplify the issue somewhat by only involving ``deterministic environments": the addition of a symbol $a$ to a prefix state $s$ results in a known prefix state $s'$. On the other hand, direct application of standard RL is problematic for three reasons. First, rewards need to be defined externally, without direct reference to training data.%
\MDEN{Maybe interesting to mention Inverse Reinforcement Learning. See for example "Between Imitation and Intention Learning, MacGlashan and Littman}
Second, they typically do not suffice for characterizing valid sequences, and need to be combined with max-likelihood training, but combination principles are not clear. Third, standard RL is an optimization framework, which tries to \emph{maximize} a reward; this is inappropriate for some (arguably all) text generation applications, for instance in language modelling, this would lead to choosing policies that would concentrate all mass on a few (perhaps a single) generated sequence(s), contrary to the very purpose of a language model, which inherently tries to approximate an underlying \emph{distribution} over sequences.   


We choose another route, which still relates to RL, but in a different sense.
We consider a class of Energy-Based Models (EBMs) \cite{lecun_tutorial_2006} that compute scores over full sequences. This class contains autoregressive models as a subclass, but the ``reward-like'' scores, being computed over the whole sequence, allow the expression of (soft) global constraints, greatly expanding the expressive power of the models.%
\MDEN{and allowing the expression of prior knowledge (?)} 
By contrast to standard RL, these scores determine (indirectly, see below) well-defined probability distributions, and can therefore, in principle, be trained by max-likelihood on the available data, avoiding the need for external reward design.%
\MDEN{Up to a point: while no external reward is imposed, the parametrization of the class of energies does involve \textit{a priori} model design choices, see section \ref{XXXX}. (put as a footnote in main text?)}
However, a serious issue with these models is that the scores they compute directly represent only \emph{unnormalized} distributions. In practice, it is often difficult to normalize these distributions, to compute the probability of a given sequence, or to sample from the model.

A key observation of this paper is that this issue can be addressed through a slight change of perspective about RL rewards and policies. Instead of trying to find a policy to \emph{optimize} a reward as in standard RL, we try to find a policy that approximates these rewards (aka energy-based scores) in a \emph{distributional} sense. These ``distributional'' policies are just the same as the standard policies, and therefore represent normalized distributions over sequences that can directly be used for sampling and evaluation, but here the objective is to find a policy that minimizes the divergence between the distribution represented by the policy and the distribution determined by the EBM, not one that maximizes the reward.%
While this change of viewpoint, from optimization to sampling, is central to our approach, the relationship with standard RL is still close and means that we can adapt RL techniques, such as Policy Gradient, as we will show.%
\MDEN{We could provide some motivation for linking optimization and sampling so closely: on the one hand, simulated annealing and $L^p$ spaces; on the other hand wll-known change of semiring in formal automata work (max-sum semiring vs. sum-times semiring)}

Our experimental exploration of these issues relies on a specific architecture for sequential EBMs, Global Autoregressive Models (GAMs), defined in \cite{gams-conll-2019-anonymised}, which we recap briefly in the next section.%
\footnote{Note to reviewers: the publication \cite{gams-conll-2019-anonymised} is scheduled to appear after the AAAI reviewing process. For this reason, for the reader's convenience, we provide a few additional details extracted from it in the \SupMat{}. We also stress differences with the current submission in the Related Work section.}

The training of these models is done in two stages. The first stage, Training-1, obtains an \emph{unnormalized} representation for the GAM that best fits the available data, in terms of sequence energies (scores). The second stage, Training-2, then tries to find a  policy that fits these energies in a distributional sense. We then make two further observations. The first one is that the final (autoregressive) policy obtained by Training-2 tends to be more sample-efficient than an inital policy obtained by standard autoregressive techniques (RNNs, etc.). The second one is that dividing the training of final policies in these two stages distinguishes two very distinct aspects of training globally-aware sequential models, where the representation produced at the end of Training-1 is relatively easy to obtain and descriptively very powerful,\MDEN{note that Training-1 can be seen as something analogous to Inverse RL.}
but where the main challenge is in moving from this representation to the final policy during Training-2.

The paper is structured as follows. The Model section  provides an overview of GAMs, motivates them in relation to Autoregressive models and Energy-based models, and explains the role of emph{a priori} features. The Training section explains the two-stage training of GAMs, with special emphasis on the connection between Training-2 and Distributional Policies. The Experiments section describes our sequence datasets, the features used and gives details on implementation. It then provides results comparing two main techniques for Training-2, Distillation and  Distributional Policy Gradient (DPG). The Conclusion recaps the main results and observations.  



==> length-features.tex <==
\subsection{Beyond Binary Features in Training-1: Length}

%\footnote{\TA{i think it is important contribution - continuous features! \MD{OK, but not clear where best to place the material, so as not to interrupt message about D-PG}}}

While the emphasis of the current paper is on Training-2 and its relationship with distributional policies in RL, we also wanted to go beyond one of the limiting assumptions of \cite{gams-conll-2019-anonymised}, namely its reliance on binary features only: e.g., presence of a substring, value of the first bit, etc. We wanted to confirm that GAMs can be applied continuous features as well, and in fact to features that have a strong inter-dependence. We also wanted to consider features that relied on weaker prior knowledge than the presence of specific motifs.

To do that, we considered an additional length feature with two components, namely $\frac{|x|}{\textrm{max\_len}} \in [0,1]$ denoted as $M$ and $\frac{|x|^2}{\textrm{max\_len}^2} \in [0,1]$ denoted as $v$. 

We note that the moments of these two features correspond to sufficient statistics for the normal distribution, and roughly speaking GAMs are obtained by matching moments of the given dataset $D$. 

We were then able during Training-1 to learn the corresponding $\lambda$ parameters using either $snis$ without modification or $rs$ with a modification for computing the upper bound (since the two components are inter-dependent).%\footnote{\TA{the only time when we modify something in training-1 comparing to CONLL}}

However, we noticed that the performance of two training setups (distillation and D-PG) was rather similar when the length feature was on or off (see \figurename~\ref{f:dpg_distill_len}). We speculate that in order to see the impact of the length feature, the strings in $D$ should be longer so that the original AM $r$ would be weaker in characterizing the length. 

      

==> main.tex <==
\input OPTRL.tex


==> related.tex <==
\section{Related Work}\label{sec:related}

GAMs have been introduced in our upcoming paper \cite{gams-conll-2019-anonymised}. While that paper already proposes the division of training in two stages, it only considers a distillation method, of limited application, for Training-2. It mentions a possible relation with RL as future work, but does not elaborate, while this is a central focus of the present submission.

Global and Energy-Based approaches to neural seq2seq models have been considered in several works. Among those, \cite{andor-etal-2016-globally} consider transition-based neural networks, and contrast local to global normalization of decision sequences, showing how the global approach avoids the \emph{label bias} problem for tasks such as tagging or parsing. Contrarily to us, they focus on inference as maximization, for instance finding the best sequence of tags for a sequence of words. \cite{Belanger:2016:SPE:3045390.3045495} address a similar class of problems (multi-labelling problems such as sequence tagging), employing an energy-based generalization of CRFs, also focussing on inference as optimization. \cite{KimBengio2016}, similar to us, consider probabilistic generative processes defined through an energy-based model. Their focus is on the generation of non-sequential objects, using GAN-type binary discriminators to train the energy representation on the available data. They do not exploit connections to RL.

Reinforcement Learning approaches for seq2seq problems have also been studied in many works. Among those, \cite{DBLP:journals/corr/RanzatoCAZ15} use an hybrid loss function to interpolate between perplexity (aka cross-entropy) training and reward optimization, with the reward being defined by evaluation measures (such as BLEU in machine translation) differing from perplexity. \cite{bahdanau_actor-critic_2016}, still in a RL-as-optimization framework, and with similar objectives, exploit an actor-critic method, where the critic (value function) helps the actor (policy) by reducing variance. \cite{Jaques-2017} and \cite{Norouzi:2016} attempt to combine log-likelihood (aka perplexity) and reward-based training in a more integrated way. In the first paper the rewards are directly defined by \emph{a priori} scores on the quality of the output, which can be computed not only at training time but also at test time. In the second paper, the way in which the rewards are integrated is done by exploiting a probabilistic formulation of rewards close to ours, but used in a different way, in particular without our notion of proposal distribution and with no explicit connection to energy-based modelling. 
In all these cases, the focus is on inference as optimization, not inference as sampling as in the present submission.

Finally, \cite{bellemare_distributional_2017} use a different notion of ``distributional RL" from ours. During policy evaluation, they replace evaluation of the \emph{mean} return from a state by the evaluation of the full \emph{distribution over returns} from that state, and define a Bellman operator for such distribution. Their goal is still to find a policy in the standard (optimization) sense, but with better robustness and stability properties.


